Energy-based discontinuous Galerkin difference methods for second-order wave equations

We combine the newly-constructed Galerkin difference basis with the energy-based discontinuous Galerkin method for wave equations in second order form. The approximation properties of the resulting method are excellent and the allowable time steps are large compared to traditional discontinuous Galerkin methods. The one drawback of the combined approach is the cost of inversion of the local mass matrix. We demonstrate that for constant coefficient problems on Cartesian meshes this bottleneck can be removed by the use of a modified Galerkin difference basis. For variable coefficients or non-Cartesian meshes this technique is not possible and we instead use the preconditioned conjugate gradient method to iteratively invert the mass matrices. With a careful choice of preconditioner we can demonstrate optimal complexity, albeit with a larger constant.

==> manuscript_table/bc_1d.tex <==
\begin{table}[htb]
\caption{Linear regression estimates of the convergence rate of $u$ and $v$ in one dimensional with Dirichlet boundary condition on the left and Neumann boundary condtion on the right.}
\label{R_bc_1d}
\begin{center}
  \begin{tabular}{|c|c c c c c|}
  \hline
Degree $(p)$ of approx. for $u$   & 1 & 3 & 5 & 7 & 9 \\
\hline
  Rate fit $u$ \text{U.-flux} &0.88& 4.20 & 6.01& 7.96 & 9.92\\
 % Rate fit $v$ \text{U.-flux} &1.31 & 3.11 & 5.23 & 7.31 & 10.81 \\
\hline
  Rate fit $u$ \text{C.-flux} &1.82 & 4.17 & 6.07& 8.05 & 10.16\\
 % Rate fit $v$ \text{C.-flux} &1.47 & 2.99 & 4.97 & 7.04 & 10.03 \\
  \hline 
  Rate fit $u$ \text{A.-flux} &0.03 & 4.04 & 5.97& 7.96 & 9.99\\
 % Rate fit $v$ \text{A.-flux} &-0.02 & 1.99 & 3.98 & 6.00 & 11.27\\
  \hline
\end{tabular}
\end{center}
\end{table}


==> manuscript_table/periodic_2d.tex <==
\begin{table}[htb]
\caption{Linear regression estimates of the convergence rate of $u$ and $v$ in two dimensional with periodic boundary condition.}\label{R_per_2d}
\begin{center}
  \begin{tabular}{|c|c c c c c|}
  \hline
Degree $(p)$ of approx. for $u$   & 1 & 3 & 5 & 7 & 9 \\
\hline
  Rate fit $u$ \text{U.-flux} &1.97 & 5.05 & 6.03& 7.78 & 8.76\\
  Rate fit $v$ \text{U.-flux} &1.37 & 3.19 & 4.99 & 7.13 & 8.96 \\
\hline
  Rate fit $u$ \text{C.-flux} &1.75 & 5.03 & 6.09& 6.87 & 8.76\\
  Rate fit $v$ \text{C.-flux} &1.36 & 3.29 & 5.22 & 7.32 & 9.27 \\
  \hline 
  Rate fit $u$ \text{A.-flux} &-2.23 & 3.65 & 5.88& 8.06 & 10.03\\
  Rate fit $v$ \text{A.-flux} &-2.17 & 1.16 & 3.78 & 6.10 & 8.30 \\
  \hline
\end{tabular}
\end{center}
\end{table}

